Harnessing the Power of Large Language Models for Natural Language to First-Order Logic Translation

Translating natural language sentences to first-order logic (NL-FOL translation) is a longstanding challenge in the NLP and formal logic literature. This paper introduces LogicLLaMA, a LLaMA-7B model fine-tuned for NL-FOL translation using LoRA on a single GPU. LogicLLaMA is capable of directly translating natural language into FOL rules, which outperforms GPT-3.5. LogicLLaMA is also equipped to correct FOL rules predicted by GPT-3.5, and can achieve similar performance as GPT-4 with a fraction of the cost. This correction ability was achieved by a novel supervised fine-tuning (SFT) + reinforcement learning with human feedback (RLHF) framework, which initially trains on synthetically perturbed NL-FOL pairs to encourage chain-of-thought reasoning and then fine-tunes with RLHF on GPT-3.5 outputs using a FOL verifier as the reward model. To train LogicLLaMA, we present MALLS (large language $\textbf{M}$odel gener$\textbf{A}$ted N$\textbf{L}$-FO$\textbf{L}$ pair$\textbf{S}$), a dataset of 34K high-quality and diverse sentence-level NL-FOL pairs collected from GPT-4. The dataset was created by implementing a pipeline that prompts GPT-4 for pairs, and dynamically adjusts the prompts to ensure the collection of pairs with rich and diverse contexts at different levels of complexity, and verifies the validity of the generated FOL rules. Codes, weights, and data are available at $\href{https://github.com/gblackout/LogicLLaMA}{{\small \text{https://github.com/gblackout/LogicLLaMA}}}$.

==> parts/algorithms.tex <==
\SetKwInput{KwInit}{Init}
\begin{algorithm}[t]
\caption{RLHF}
\SetAlgoLined
\KwIn{Reward Model $RM$, NL-perturbed-FOL-rule pairs $\cD = \{\anB{\vx, \vx_{\hat{R}}}_i\}_{i=1}^n$}
\KwInit{The remote $GPT$, Actor $\pi_\theta$ and critic $C_\omega$, experience set $\cE=\emptyset$}

\While{True}{

    \BlankLine

    \tcp{Make experience}
    \For{$i=1\to N$}{
        Sample $\vx, \vx_{\hat{R}} \sim \cD $
        
        Take actions $A = \{a_1, a_2, .., a_T\} \gets \pi_\theta(a_t|\vx, \vx_{\hat{R}})$

        \BlankLine
        \BlankLine
        
        Concatenate the prompts $\vx^* \gets \vx + \vx_{\hat{R}} + A$

        Get response $\vx_R \gets GPT(\vx^*)$

        Parse the rule $R \gets Parser(\vx_R)$

        \BlankLine
        \BlankLine

        \tcp{Only one reward for the whole episode!}
        Get reward $r \gets RM(R)$
        
        \tcp{Estimate the value only for the last action!}
        Last state $s_T \gets \vx + \vx_{\hat{R}} + A_{<T}$
        
        Get value estimates $v = C_\omega(a_T|s_T)$
        
        Compute advantage $adv = r - v$

        \BlankLine
        \BlankLine
        
        Add experience $\cE.add\brB{\anB{s_T, A, r, v, adv}}$
    }

    \BlankLine
    \BlankLine

    \tcp{Policy gradient update on $\pi_\theta$}
    Update $\theta$ with $\nabla \sum_i^N \log \pi_\theta(A|\vx, \vx_{\hat{R}}) * adv_i$

    \BlankLine

    \tcp{Square loss update on $C_\omega$}
    Update $\omega$ with $\nabla \sum_i^N \brB{r_i - v_i}^2$
}


\label{algo:overview}
\end{algorithm}

==> parts/main-res-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{BLEU and the logical equivalence (LE) scores of \method and GPT models on the FOLIO datasets. Direction translation using \method achieves better performance than GPT3.5 and CoT correction achieves similar performance as 5-shot GPT4.}
\label{tab:main-res-table}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multirow{3}{*}{Metrics}     & \multicolumn{9}{c}{FOLIO}                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\
                             & \multicolumn{4}{c}{GPT}                                                                                                                                                                                                           &  & \multicolumn{4}{c}{\method}                                                                                                                                                                                                                          \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
                             & \begin{tabular}[c]{@{}c@{}}GPT3.5\\ 0-shot\end{tabular} & \begin{tabular}[c]{@{}c@{}}GPT3.5\\ 5-shot\end{tabular} & \begin{tabular}[c]{@{}c@{}}GPT4\\ 0-shot\end{tabular} & \begin{tabular}[c]{@{}c@{}}GPT4\\ 5-shot\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Direct\\ Translation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Naive\\ Correction\end{tabular} & \begin{tabular}[c]{@{}c@{}}CoT\\ Correction\end{tabular} & \begin{tabular}[c]{@{}c@{}}CoT\\ Correction RLHF\end{tabular} \\ \midrule
\multicolumn{1}{l}{FOL BLEU} & 0.248                                                   & 0.341                                                   & 0.372                                                 & 0.400                                                 &  & 0.372                                                        & 0.373                                                      & 0.332                                                    & 0.386                                                         \\
\multicolumn{1}{l}{FOL LE}   & 0.429                                                   & 0.767                                                   & 0.799                                                 & 0.855                                                 &  & 0.818                                                        & 0.840                                                      & 0.730                                                    & 0.849                                                         \\ \bottomrule
\end{tabular}%
}
\end{table}

==> parts/perturb-operations-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{The list of all atomic perturbations.}
\label{tab:perturb-operations}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
\multicolumn{1}{c}{Operation Type} & \multicolumn{1}{c}{Subtypes} & \multicolumn{1}{c}{Original}                             & \multicolumn{1}{c}{Perturbed}                     \\ \midrule
\multirow{4}{*}{Label Change}      & Change Predicate             & $\tblue{P}(A) \land R(B)$                                & $\tred{R}(A) \land R(B)$                          \\
                                   & \multirow{2}{*}{Change Term} & \multirow{2}{*}{$\forall \tblue{x}\;\; P(x) \land P(B)$} & $\forall \tred{y} \;\; P(x) \land P(B)$           \\
                                   &                              &                                                          & $\forall x \;\; P(x) \land P(\tred{x})$     \\
                                   & Change Operator              & $\forall x \;\; P(x) \;\tblue{\land}\; P(B)$                 & $\forall x \;\; P(x) \;\tred{\lor}\; P(B)$            \\ \midrule
\multirow{4}{*}{Insert}            & \multirow{2}{*}{Insert Term} & \multirow{2}{*}{$\forall x \;\; P(x) \land P(B)$}        & $\forall x \; \tred{\exists y} \;\; P(x) \land P(B)$ \\
                                   &                              &                                                          & $\forall x \;\; P(x) \land P(\tred{x, }\;B)$        \\
                                   & Insert Negation              & $P(A) \land P(B) \land P(C)$                             & $P(A) \land \tred{\neg(}P(B) \land P(C)\tred{)}$  \\
                                   & Insert  Formula              & $P(A) \land P(B)$                                        & $P(A) \land P(B) \;\tred{\to R(C)}$                 \\ \midrule
\multirow{4}{*}{Delete}            & \multirow{2}{*}{Delete Term} & $\tblue{\forall x} \; \forall y \;\; P(x) \land R(x, y)$ & $\forall y \;\; P(x) \land R(x, y)$               \\
                                   &                              & $\forall x \; \forall y \;\; P(x) \land R(\tblue{x, }\;y)$ & $\forall x \; \forall y \;\; P(x) \land R(y)$     \\
                                   & Delete Negation              & $\tblue{\neg(}P(A) \land P(B)\tblue{)}$                  & $\neg(P(A) \land P(B))$                           \\
                                   & Delete Formula               & $P(A) \;\tblue{\land}\; \tblue{P(B)}\; \land P(C)$                     & $P(A) \land P(C)$                                 \\ \bottomrule
\end{tabular}%
}
\end{table}
